Can Large Language Models Write Parallel Code?

Large language models are increasingly becoming a popular tool for software development. Their ability to model and generate source code has been demonstrated in a variety of contexts, including code completion, summarization, translation, and lookup. However, they often struggle to generate code for complex programs. In this paper, we study the capabilities of state-of-the-art language models to generate parallel code. In order to evaluate language models, we create a benchmark, ParEval, consisting of prompts that represent 420 different coding tasks related to scientific and parallel computing. We use ParEval to evaluate the effectiveness of several state-of-the-art open- and closed-source language models on these tasks. We introduce novel metrics for evaluating the performance of generated code, and use them to explore how well each large language model performs for 12 different computational problem types and six different parallel programming models.

==> Makefile <==
MAIN=paper

FIGS = $(wildcard figs/*.png)

LATEXFLAGS += --shell-escape

all: $(MAIN).pdf

$(MAIN).pdf: $(wildcard *.tex) $(wildcard *.tikz) $(FIGS)
	pdflatex $(LATEXFLAGS) $(MAIN)
	bibtex $(MAIN)
	pdflatex $(LATEXFLAGS) $(MAIN)
	pdflatex $(LATEXFLAGS) $(MAIN)

figs: $(FIGS)
	$(MAKE) -C figs

clean:
	$(RM) *.aux *.log $(MAIN).dvi $(MAIN).ps $(MAIN).pdf $(MAIN).bbl $(MAIN).blg $(MAIN).synctex.gz comment.cut paper.out

findref:
	@echo
	@test \
          `grep -c undefined $(MAIN).log | grep -v There | sed 's/.*\`//g' | sed "s/'.*//g"` = "0" \
            && echo "No undefined references" \
            || echo Finding undefined references ; \
               for uref in `grep undefined $(MAIN).log | grep -v There | sed 's/.*\`//g' | sed "s/'.*//g"`; \
               do  \
                echo "--> $$uref ";\
                grep -n "[rc][ei].*$$uref" *.tex | grep -v '.tex:[0-9]*:%' | sed 's/:/ -- Line /' | sed 's/:/:  /';\
                echo ;\
               done

.PHONY: clean figs


==> problems.tex <==
\begin{table}[]
    \begin{tabular}{@{}lll@{}}
    \toprule
    Problem Name                                  & Problem Type & Description                                                                                                                                                                       \\ \midrule
    LU Decomp                                     & Dense LA     & LU factorize a matrix                                                     \\
    Solve                                         & Dense LA     & Solve a linear system Ax=b for x                                                                                   \\
    GeMM                                          & Dense LA     & Dense matrix multiplication                                                       \\
    AXPY                                          & Dense LA     & Compute z = alpha*x+y where x, y, and z are vectors                                                                                                           \\
    GeMV                                          & Dense LA     & Dense matrix vector multiplication                         \\
    Inverse FFT                                   & FFT          & In-place inverse fourier transform                                                                                                                              \\
    DFT                                           & FFT          & Discrete fourier transform                                                                                                       \\
    FFT Conjugate                                 & FFT          & In-place fourier transform with conjugate outputs                                                                                        \\
    Split FFT                                     & FFT          & Fourier transform with separate real and imaginary outputs                                       \\
    FFT Out Of Place                              & FFT          & Out-of-place fourier transform                                                                                         \\
    Convex hull                                   & Geometry     & Find convex hull                                    \\
    Convex Hull Perimeter                         & Geometry     & Compute perimeter of convex hull                                                                            \\
    Smallest Triangle                             & Geometry     & Area of the smallest triangle that can be formed by any 3 points                                                                                                      \\
    Closest Pair 2D                               & Geometry     & Distance between the closest two points                                                                                                         \\
    Closest Pair 1D                               & Geometry     & Distance between the closest two elements                                                                                                             \\
    Edge Count                                    & Graph        & Count the number of edges in a directed graph                                                   \\
    Largest Component                             & Graph        & Vertices count of the largest component of an undirected graph                   \\
    Highest Degree                                & Graph        & Highest vertex degree in a undirected graph                           \\
    Count Components                              & Graph        & Number of connected components in an undirected graph                                \\
    Shortest Path                                 & Graph        & Shortest path length between two vertices             \\
    Pixel Histogram                               & Histogram    & Count the number of pixels in image with each grayscale intensity. The vector `image` is a grayscale image with values 0-255. Store the results in `bins`.                        \\
    Bin 0-100                                     & Histogram    & Vector x contains values between 0 and 100, inclusive. Count the number of values in {[}0,10), {[}10, 20), {[}20, 30), ... and store the counts in `bins`.                        \\
    Count Quadrants                               & Histogram    & Count the number of cartesian points in each quadrant. The vector points contains a list of `Point` objects. Store the counts in `bins`.                                          \\
    First Letter Counts                           & Histogram    & For each letter in the alphabet, count the number of strings in the vector s that start with that letter. Assume all strings are in lower case. Store the output in `bins` array. \\
    Count Quartile                                & Histogram    & Count the number of doubles in the vector x that have a fractional part in {[}0, 0.25), {[}0.25, 0.5), {[}0.5, 0.75), and {[}0.75, 1). Store the counts in `bins`.                \\
    XOR                                           & Reduce       & Return the logical XOR reduction of the vector of bools x.                                                                                                                        \\
    Product of Inverses                           & Reduce       & Return the product of the vector x with every odd indexed element inverted.                                                                                                       \\
    Average                                       & Reduce       & Compute the average of the vector x.                                                                                                                                              \\
    Smallest odd number                           & Reduce       & Return the value of the smallest odd number in the vector x.                                                                                                                      \\
    Sum of min of pairs                           & Reduce       & Return the sum of the minimum value at each index of vectors x and y for all indices. i.e. sum = min(x\_0, y\_0) + min(x\_1, y\_1) + min(x\_2, y\_2) + ...                        \\
    Prefix Sum                                    & Scan         & Compute the prefix sum of the vector x into output.                                                                                                                               \\
    Scan with min function                        & Scan         & Replace the i-th element of the vector x with the minimum value from indices 0 through i.                                                                                         \\
    Sum of prefix sum array                       & Scan         & Compute the prefix sum array of the vector x and return its sum.                                                                                                                  \\
    Reverse prefix sum                            & Scan         & Compute the reverse prefix sum of the vector x into output.                                                                                                                       \\
    Largest contiguous subarray sum               & Scan         & Return the largest sum of any contiguous subarray in the vector x.                                                                                                                \\
    Search for last struct by key                 & Search       & Return the index of the last Book item in the vector books where Book.pages is less than 100.                                                                                     \\
    Check if array contains value                 & Search       & Return true if the vector x contains the value `target`. Return false otherwise.                                                                                                  \\
    Find the closest number to pi                 & Search       & Return the index of the value in the vector x that is closest to the math constant PI. Use M\_PI for the value of PI.                                                             \\
    Find the first even number                    & Search       & Return the index of the first even number in the vector x.                                                                                                                        \\
    XOR Contains                                  & Search       & Return true if `val` is only in one of vectors x or y. Return false if it is in both or neither.                                                                                  \\
    Sort complex numbers by magnitude             & Sort         & Sort the vector x of complex numbers by their magnitude in ascending order.                                                                                                       \\
    k-th Smallest Element                         & Sort         & Given a vector x and an int k find the k-th smallest element of x                                                                                                                 \\
    Sorted Ranks                                  & Sort         & For each value in the vector x compute its index in the sorted vector. Store the results in `ranks`.                                                                              \\
    Sort an array of structs by key               & Sort         & Sort an array of structs by some property of the struct.                                                                                                                          \\
    Sort non-zero elements                        & Sort         & Sort the vector x in ascending order ignoring elements with value 0. Leave zero valued elements in-place.                                                                         \\
    Sparse Solve                                  & Sparse LA    & Solve the sparse linear system Ax=b for x. A is a sparse NxN matrix in COO format. x and b are dense vectors with N elements.                                                     \\
    SpMM                                          & Sparse LA    & Compute the sparse matrix multiplication Y=AX. A is the MxK matrix, X is the KxN matrix, and Y is the MxN matrix.                                                                 \\
    SpMV                                          & Sparse LA    & Compute y = alpha*A*x + beta*y where alpha and beta are scalars, x and y are vectors, and A is a sparse matrix stored in COO format.                                              \\
    Sparse AXPY                                   & Sparse LA    & Compute z = alpha*x+y where x and y are sparse vectors. Store the result in z.                                                                                                    \\
    Sparse LU Decomp                              & Sparse LA    & Factorize a sparse NxN matrix stored in COO format into A=LU where L is a lower triangular matrix and U is an upper triangular matrix.                                            \\
    XOR Kernel                                    & Stencil      & Set every cell's value to 1 if it has exactly one neighbor that's a 1. Otherwise set it to 0.                                                                                     \\
    Edge Kernel                                   & Stencil      & Apply edge kernel to grayscale image                                                                                                                                              \\
    1d Jacobi 3-point stencil                     & Stencil      & Compute one iteration of 1D jacobi with a 3-point stencil.                                                                                                                        \\
    2d Jacobi 5-point stencil                     & Stencil      & Compute one iteration of 2D jacobi with a 5-point stencil.                                                                                                                        \\
    Game Of Life                                  & Stencil      & Simulate one generation of Game of Life. Cells are marked live or dead.                                                                                                           \\
    ReLU                                          & Transform    & Compute the ReLU function on every element of x. Elements less than zero become zero, while elements greater than zero stay the same.                                             \\
    Negate Odds                                   & Transform    & In the vector x negate the odd values and divide the even values by 2.                                                                                                            \\
    Inverse Offset                                & Transform    & Replace every element of the vector x with 1-1/x.                                                                                                                                 \\
    Squaring                                      & Transform    & Replace every element of x with the square of its value.                                                                                                                          \\
    Map Function                                  & Transform    & Apply a function to every value in x and store the results                                                                                                                        \\ \bottomrule
    \end{tabular}
    \end{table}

